CIRCLE: Capture In Rich Contextual Environments

Synthesizing 3D human motion in a contextual, ecological environment is important for simulating realistic activities people perform in the real world. However, conventional optics-based motion capture systems are not suited for simultaneously capturing human movements and complex scenes. The lack of rich contextual 3D human motion datasets presents a roadblock to creating high-quality generative human motion models. We propose a novel motion acquisition system in which the actor perceives and operates in a highly contextual virtual world while being motion captured in the real world. Our system enables rapid collection of high-quality human motion in highly diverse scenes, without the concern of occlusion or the need for physical scene construction in the real world. We present CIRCLE, a dataset containing 10 hours of full-body reaching motion from 5 subjects across nine scenes, paired with ego-centric information of the environment represented in various forms, such as RGBD videos. We use this dataset to train a model that generates human motion conditioned on scene information. Leveraging our dataset, the model learns to use ego-centric scene information to achieve nontrivial reaching tasks in the context of complex 3D scenes. To download the data please visit https://stanford-tml.github.io/circle_dataset/.

==> defs.tex <==
%% editing comment

\newcommand{\cmt}[1]{\textcolor{red}{\textbf {#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\karen}[1]{\textcolor{red}{[Karen: #1]}}
\newcommand{\danNote}[1]{\textcolor{blue}{[#1]}}
\newcommand{\fig}[1]{Figure~\ref{#1}}

%% spacing around titles
\usepackage[small,compact]{titlesec}
%\titlespacing*{\section}{0pt}{6pt plus 2pt minus 2pt}{3pt plus 1pt minus 1pt}
%\titlespacing*{\subsection}{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing*{\subsubsection}{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing*{\paragraph}{0pt}{1pt plus 2pt minus 2pt}{10pt}

%% spacing around lists
\usepackage{enumitem}
\setlist[itemize]{itemsep=0pt, topsep=0pt, leftmargin=25pt}
\setlist[enumerate]{itemsep=0pt, topsep=0pt, leftmargin=15pt}

%% ignore text
\long\def\ignorethis#1{}

%% abbreviations
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\iid{i.i.d\onedot}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{et al\onedot}
\makeatother
\def\shortcite{\def\citename##1{}\@internalcite}

%% reference shortcuts
\newcommand{\figtodo}[1]{\framebox[0.8\columnwidth]{\rule{0pt}{1in}#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}

%% FA COMMANDS
\setlength{\fboxsep}{1em}
\newcommand{\spacecont}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\spacedisc}[1]{\ensuremath{\mathit{#1}}}

%% frequently used mathematical structures
\newcommand{\vc}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\pd}[2]{\ensuremath{\frac{\partial{#1}}{\partial{#2}}}}
\newcommand{\pdd}[3]{\ensuremath{\frac{\partial^2{#1}}{\partial{#2}\,\partial{#3}}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}

% math macros
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\matr}[1]{\bm{#1}}
\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\vdot}[1]{\dot{\vect{#1}}}
\newcommand{\vddot}[1]{\ddot{\vect{#1}}}

% Local Variables:
% TeX-master: "paper"
% End:

